Optimal Edge Caching For Individualized Demand Dynamics

The ever-growing end user data demands, and the simultaneous reductions in memory costs are fueling edge-caching deployments. Caching at the edge is substantially different from that at the core and needs to take into account the nature of individual data demands. For example, an individual user may not be interested in requesting the same data item again, if it has recently requested it. Such individual dynamics are not apparent in the aggregated data requests at the core and have not been considered in popularity-driven caching designs for the core. Hence, these traditional caching policies could induce significant inefficiencies when applied at the edges. To address this issue, we develop new edge caching policies optimized for the individual demands that also leverage overhearing opportunities at the wireless edge. With the objective of maximizing the hit ratio, the proposed policies will actively evict the data items that are not likely to be requested in the near future, and strategically bring them back into the cache through overhearing when they are likely to be popular again. Both theoretical analysis and numerical simulations demonstrate that the proposed edge caching policies could outperform the popularity-driven policies that are optimal at the core.

==> acknowledgment.tex <==
\section*{Acknowledgments}
This should be a simple paragraph before the References to thank those individuals and institutions who have supported your work on this article.

==> test.tex <==
\section{Introduction}
%   \IEEEPARstart{T}{his} file is intended to serve as a ``sample article file''
%   for IEEE journal papers produced under \LaTeX\ using
%   IEEEtran.cls version 1.8b and later. The most common elements are covered in the simplified and updated instructions in ``New\_IEEEtran\_how-to.pdf''. For less common elements you can refer back to the original ``IEEEtran\_HOWTO.pdf''. It is assumed that the reader has a basic working knowledge of \LaTeX. Those who are new to \LaTeX \ are encouraged to read Tobias Oetiker's ``The Not So Short Introduction to \LaTeX ,'' available at: \url{http://tug.ctan.org/info/lshort/english/lshort.pdf} which provides an overview of working with \LaTeX.
  

% Caching techniques are widely used to provide fast
% data retrievals.  
With ever reducing memory costs coupled with 
explosive data demands at the network edges
that are driven by the internet of things, edge computing and 5G, 
% caching capabilities are spread out from the network
% core to the edges 
edge caching is becoming increasingly prevalent
for supporting fast data 
retrieval~\cite{qian2012web, 
niyato2016novel, wang2014cache, zhang2018cooperative}.
Although extensive 
studies~\cite{jia2017efficient,li2016popularity, 
huang2013analysis, cidon2015dynacache} 
have been conducted 
to optimize caching strategies 
for relatively stationary data demands at the network core, 
caching at the edges has substantially distinctions than that at the core
due to individualized demand dynamics,
and therefore should be studied in their own right.  
% these results cannot be directly applied for the edge caching
% where the data demands are highly individualized. 
In this paper, we will propose new caching policies 
optimized for the individualized data demands at the wireless edges. 

\subsection{Challenge: Individualized Demands at Network Edges}
At the network core, 
data demands are aggregated from 
a large number of end-users.
Thus, the demand dynamics of each individual user 
could become negligible, which leads to 
relatively stationary data popularities for the population.
% data requests are typically assumed to be generated 
% from a popularity distribution which evolves relatively slowly.
A number of popularity-driven policies have been 
proposed for optimizing caching 
at the core~\cite{li2016popularity,jiang2002lirs}. 
% In real systems where the popularities are unknown, 
% historical request information is used to estimate the data popularities 
% and guide the caching decision. 
Inspired by the observation that data items recently requested by one user 
are very likely to be requested again by others with similar interests, 
the Least Recently used (LRU) policy
estimates the popularity by the data recency 
and caches the most recently requested data items. 
% The LRU policy and its variants have been widely implemented at the core,
% and validated to achieve considerably good 



  The templates are intended to {\bf{approximate the final look and page length of the articles/papers}}. {\bf{They are NOT intended to be the final produced work that is displayed in print or on IEEEXplore\textsuperscript{\textregistered}}}. They will help to give the authors an approximation of the number of pages that will be in the final version. The structure of the \LaTeX\ files, as designed, enable easy conversion to XML for the composition systems used by the IEEE. The XML files are used to produce the final print/IEEEXplore pdf and then converted to HTML for IEEEXplore.
  
  The following online groups are helpful to beginning and experienced \LaTeX\ users. A search through their archives can provide many answers to common questions.
  \begin{list}{}{}
  \item{\url{http://www.latex-community.org/}} 
  \item{\url{https://tex.stackexchange.com/} }
  \end{list}
  
  See \cite{ref1,ref2,ref3,ref4,ref5} for resources on formatting math into text and additional help in working with \LaTeX .
  
  For some of the remainer of this sample we will use dummy text to fill out paragraphs rather than use live text that may violate a copyright.
  
  Itam, que ipiti sum dem velit la sum et dionet quatibus apitet voloritet audam, qui aliciant voloreicid quaspe volorem ut maximusandit faccum conemporerum aut ellatur, nobis arcimus.
  Fugit odi ut pliquia incitium latum que cusapere perit molupta eaquaeria quod ut optatem poreiur? Quiaerr ovitior suntiant litio bearciur?
  
  Onseque sequaes rectur autate minullore nusae nestiberum, sum voluptatio. Et ratem sequiam quaspername nos rem repudandae volum consequis nos eium aut as molupta tectum ulparumquam ut maximillesti consequas quas inctia cum volectinusa porrum unt eius cusaest exeritatur? Nias es enist fugit pa vollum reium essusam nist et pa aceaqui quo elibusdandis deligendus que nullaci lloreri bla que sa coreriam explacc atiumquos simolorpore, non prehendunt lam que occum\cite{ref6} si aut aut maximus eliaeruntia dia sequiamenime natem sendae ipidemp orehend uciisi omnienetus most verum, ommolendi omnimus, est, veni aut ipsa volendelist mo conserum volores estisciis recessi nveles ut poressitatur sitiis ex endi diti volum dolupta aut aut odi as eatquo cullabo remquis toreptum et des accus dolende pores sequas dolores tinust quas expel moditae ne sum quiatis nis endipie nihilis etum fugiae audi dia quiasit quibus.
  \IEEEpubidadjcol
  Ibus el et quatemo luptatque doluptaest et pe volent rem ipidusa eribus utem venimolorae dera qui acea quam etur aceruptat.
  Gias anis doluptaspic tem et aliquis alique inctiuntiur?
  
  Sedigent, si aligend elibuscid ut et ium volo tem eictore pellore ritatus ut ut ullatus in con con pere nos ab ium di tem aliqui od magnit repta volectur suntio. Nam isquiante doluptis essit, ut eos suntionsecto debitiur sum ea ipitiis adipit, oditiore, a dolorerempos aut harum ius, atquat.
  
  Rum rem ditinti sciendunti volupiciendi sequiae nonsect oreniatur, volores sition ressimil inus solut ea volum harumqui to see\eqref{deqn_ex1a} mint aut quat eos explis ad quodi debis deliqui aspel earcius.
  
  \begin{equation}
  \label{deqn_ex1a}
  x = \sum_{i=0}^{n} 2{i} Q.
  \end{equation}
  
  Alis nime volorempera perferi sitio denim repudae pre ducilit atatet volecte ssimillorae dolore, ut pel ipsa nonsequiam in re nus maiost et que dolor sunt eturita tibusanis eatent a aut et dio blaudit reptibu scipitem liquia consequodi od unto ipsae. Et enitia vel et experferum quiat harum sa net faccae dolut voloria nem. Bus ut labo. Ita eum repraer rovitia samendit aut et volupta tecupti busant omni quiae porro que nossimodic temquis anto blacita conse nis am, que ereperum eumquam quaescil imenisci quae magnimos recus ilibeaque cum etum iliate prae parumquatemo blaceaquiam quundia dit apienditem rerit re eici quaes eos sinvers pelecabo. Namendignis as exerupit aut magnim ium illabor roratecte plic tem res apiscipsam et vernat untur a deliquaest que non cus eat ea dolupiducim fugiam volum hil ius dolo eaquis sitis aut landesto quo corerest et auditaquas ditae voloribus, qui optaspis exero cusa am, ut plibus.
  
  
  \section{Some Common Elements}
  \subsection{Sections and Subsections}
  Enumeration of section headings is desirable, but not required. When numbered, please be consistent throughout the article, that is, all headings and all levels of section headings in the article should be enumerated. Primary headings are designated with Roman numerals, secondary with capital letters, tertiary with Arabic numbers; and quaternary with lowercase letters. Reference and Acknowledgment headings are unlike all other section headings in text. They are never enumerated. They are simply primary headings without labels, regardless of whether the other headings in the article are enumerated. 
  
  \subsection{Citations to the Bibliography}
  The coding for the citations is made with the \LaTeX\ $\backslash${\tt{cite}} command. 
  This will display as: see \cite{ref1}.
  
  For multiple citations code as follows: {\tt{$\backslash$cite\{ref1,ref2,ref3\}}}
   which will produce \cite{ref1,ref2,ref3}. For reference ranges that are not consecutive code as {\tt{$\backslash$cite\{ref1,ref2,ref3,ref9\}}} which will produce  \cite{ref1,ref2,ref3,ref9}
  
  \subsection{Lists}
  In this section, we will consider three types of lists: simple unnumbered, numbered, and bulleted. There have been many options added to IEEEtran to enhance the creation of lists. If your lists are more complex than those shown below, please refer to the original ``IEEEtran\_HOWTO.pdf'' for additional options.\\
  
  \subsubsection*{\bf A plain  unnumbered list}
  \begin{list}{}{}
  \item{bare\_jrnl.tex}
  \item{bare\_conf.tex}
  \item{bare\_jrnl\_compsoc.tex}
  \item{bare\_conf\_compsoc.tex}
  \item{bare\_jrnl\_comsoc.tex}
  \end{list}
  
  \subsubsection*{\bf A simple numbered list}
  \begin{enumerate}
  \item{bare\_jrnl.tex}
  \item{bare\_conf.tex}
  \item{bare\_jrnl\_compsoc.tex}
  \item{bare\_conf\_compsoc.tex}
  \item{bare\_jrnl\_comsoc.tex}
  \end{enumerate}
  
  \subsubsection*{\bf A simple bulleted list}
  \begin{itemize}
  \item{bare\_jrnl.tex}
  \item{bare\_conf.tex}
  \item{bare\_jrnl\_compsoc.tex}
  \item{bare\_conf\_compsoc.tex}
  \item{bare\_jrnl\_comsoc.tex}
  \end{itemize}
  
  
  
  
  
  \subsection{Figures}
  Fig. 1 is an example of a floating figure using the graphicx package.
   Note that $\backslash${\tt{label}} must occur AFTER (or within) $\backslash${\tt{caption}}.
   For figures, $\backslash${\tt{caption}} should occur after the $\backslash${\tt{includegraphics}}.
  
  \begin{figure}[!t]
  \centering
  \includegraphics[width=2.5in]{fig1}
  \caption{Simulation results for the network.}
  \label{fig_1}
  \end{figure}
  
  Fig. 2(a) and 2(b) is an example of a double column floating figure using two subfigures.
   (The subfig.sty package must be loaded for this to work.)
   The subfigure $\backslash${\tt{label}} commands are set within each subfloat command,
   and the $\backslash${\tt{label}} for the overall figure must come after $\backslash${\tt{caption}}.
   $\backslash${\tt{hfil}} is used as a separator to get equal spacing.
   The combined width of all the parts of the figure should do not exceed the text width or a line break will occur.
  %
  \begin{figure*}[!t]
  \centering
  \subfloat[]{\includegraphics[width=2.5in]{fig1}%
  \label{fig_first_case}}
  \hfil
  \subfloat[]{\includegraphics[width=2.5in]{fig1}%
  \label{fig_second_case}}
  \caption{Dae. Ad quatur autat ut porepel itemoles dolor autem fuga. Bus quia con nessunti as remo di quatus non perum que nimus. (a) Case I. (b) Case II.}
  \label{fig_sim}
  \end{figure*}
  
  Note that often IEEE papers with multi-part figures do not place the labels within the image itself (using the optional argument to $\backslash${\tt{subfloat}}[]), but instead will
   reference/describe all of them (a), (b), etc., within the main caption.
   Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
   labels, the optional argument to $\backslash${\tt{subfloat}} must be present. If a
   subcaption is not desired, leave its contents blank,
   e.g.,$\backslash${\tt{subfloat}}[].
